StarAI: Reducing incompleteness in the game of Bridge using PLP

Bridge is a trick-taking card game requiring the ability to evaluate probabilities since it is a game of incomplete information where each player only sees its cards. In order to choose a strategy, a player needs to gather information about the hidden cards in the other players' hand. We present a methodology allowing us to model a part of card playing in Bridge using Probabilistic Logic Programming.

==> conclusion.tex <==
Bridge is the right field to test the state-of-the-art techniques and to develop new tools of AI. For example, teaching computers to dynamically evaluate one's hand may need techniques from statistical learning. Inductive logic programming can be naturally applied to learn bidding and leading rules from existing human playing examples. Planner based on probabilistic logic programming could be developed for constructing game playing agents that can exploit expert knowledge of bridge encoded as logic formulas and that are able to explain their actions in human understandable languages. The success of these experiments may enable us to build intelligent systems that can work in multiple different domains.
